Teaching Interaction using State Diagrams

To make computational thinking appealing to young learners, initial programming instruction looks very different now than a decade ago, with increasing use of graphics and robots both real and virtual. After the first steps, children want to create interactive programs, and they need a model for this. State diagrams provide such a model. This paper documents the design and implementation of a Model-Driven Engineering tool, SD Draw, that allows even primary-aged children to draw and understand state diagrams, and create modifiable app templates in the Elm programming language using the model-view-update pattern standard in Elm programs. We have tested this with grade 4 and 5 students. In our initial test, we discovered that children quickly understand the motivation and use of state diagrams using this tool, and will independently discover abstract states even if they are only taught to model using concrete states. To determine whether this approach is appropriate for children of this age we wanted to know: do children understand state diagrams, do they understand the role of reachability, and are they engaged by them? We found that they are able to translate between different representations of state diagrams, strongly indicating that they do understand them. We found with confidence p<0.001 that they do understand reachability by refuting the null hypothesis that they are creating diagrams randomly. And we found that they were engaged by the concept, with many students continuing to develop their diagrams on their own time after school and on the weekend.

==> eptcsdata.tex <==
\providecommand{\firstpage}{132}
\providecommand{\publicationstatus}{P. Achten \& E. Machkasova  (Eds.): Trends in\\
Functional Programming in Education (TFPIE) 2021/22
\\
EPTCS 363, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.363.8}{10.4204/EPTCS.363.8}}
\pdfoutput=1

